Superradiant amplification by stars and black holes

In this thesis we study the phenomenon of superradiance and its implications to the stability of black-holes (BH) and perfect-fluid stars. Superradiance is a radiation enhancement process that involves rotating dissipative systems. In BH spacetimes, superradiance is due to dissipation at the event horizon, with interesting associated phenomena, namely floating orbits and BH-bombs. BH superradiance is a very interdisciplinary topic, and its study allows us to obtain important results in the area of particle physics. The scattering of a scalar field by a rotating BH leads to the formation of quasi-boundstates. In rotational systems, these states can give rise to superradiant instabilities. These results were recently used to impose constraints to the mass of fundamental particles and darkmatter candidates. In this work, it is shown that, when dissipation is properly included, similar results are achievable in self-gravitating systems other than black-holes, such as perfect fluid stars. It is also demonstrated that the relativistic effects related to the phenomenon of frame-dragging are neglectable in this calculation.

==> Thesis_Chapter2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                      %
%     File: Thesis_Introduction.tex                                    %
%     Tex Master: Thesis.tex                                           %
%                                                                      %
%     Author: Andre C. Marta                                           %
%     Last modified : 28 Feb 2014                                      %
%                                                                      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{Derivation of the Klein-Gordon equation}
\label{chapter:introduction}

The Einstein's vacuum equations can be obtained by applying the variational method to the Einstein-Hilbert action. To study a perturbation, one must couple this action to a field that describes it before obtaining the equations of motion. This perturbation, which consists of a small deviation of the background geometry, is also described by an equation of motion and the solution of this equation dictates the stability of the system against that perturbation. Notice that the perturbation must be small because otherwise we would no longer be working in the same initial background geometry. In this chapter, the equation of motion for a massive complex scalar field is deduced. 

Since we are studying a scalar perturbation, we shall minimally couple the action to a massive scalar field $\Psi$:
\be
S=\int_\Omega\mathcal{L}d\Omega=\int_\Omega \sqrt{-g}\left[\frac{R}{\kappa}-\frac{1}{2}g^{ab}\partial_a\Psi^*\partial_b\Psi-\frac{\mu^2}{2}\Psi^*\Psi\right]d\Omega,
\ee
where $R$ is the Ricci's scalar, $\kappa$ is the coupling constant, $\mu^2$ is the mass of the scalar field, $g_{ab}$ is the metric tensor, and $g$ is the metric determinant.

The equations of motion for a given field are obtained by minimizing the action, that is, differentiating the action in order to the field in study and equaling the result to zero:
\be
\label{variat}
\delta S=\int_\Omega\left(\frac{\partial\mathcal{L}}{\partial\Psi}\delta\Psi\right) d\Omega = 0.
\ee

We shall differentiate in order to $\Psi^*$ to obtain directly an equation of motion for $\Psi$. Applying the previous method to the action given we obtain
\be
\int_\Omega \sqrt{-g} \left(-\frac{1}{2}g^{ab}\partial_b \Psi \partial_a \delta\Psi^* -\frac{\mu^2}{2}\Psi\delta\Psi^*\right)d\Omega=0.
\ee

The second term in the integral is already written in the form \eqref{variat}, but the first term still deppends on the derivative of our field. Integrating that term by parts we obtain
\be
\int_\Omega \left[ \frac{1}{2} \partial_a \left(\sqrt{-g} g^{ab} \partial_b \Psi\right) - \sqrt{-g} \frac{\mu^2}{2}\Psi\right] \delta\Psi^* d\Omega = 0,
\ee
since the integral at the boundary of $\Omega$, the infinity, is equal to zero. This happens because we will be working with asymptotically flat solutions of the Einstein field equations. Since this equation must hold for an arbitrary scalar field $\Psi^*$, the function inside the integral must be identically zero from which we obtain
\be
\frac{1}{\sqrt{-g}}\partial_a \left(\sqrt{-g} g^{ab} \partial_b \Psi\right)=\mu^2\Psi.
\ee

Now, to write the left side of the previous result in a covariant description, note that $\Psi$ is a scalar field, and therefore its partial derivative is equal to the covariant derivative. Furthermore, using the fact that $\partial_a\sqrt{-g}=\Gamma^b_{ba}\sqrt{-g}$, the product derivative of this term can be written in the form
\be
\frac{1}{\sqrt{-g}}\partial_a \left(\sqrt{-g} g^{ab} \nabla_b \Psi\right)=\Gamma^b_{ba}\nabla^a\Psi+\partial_a\nabla^a\Psi,
\ee
and using the definition for the covariant derivative of a rank-1 covariant tensor we obtain 
\be
\nabla_a\nabla^a\Psi=\mu^2\Psi,
\ee
which is the Klein-Gordon equation for the scalar field $\Psi$ that we were trying to obtain.


\cleardoublepage


